Asymptotic Properties of Primal-Dual Algorithm for Distributed Stochastic Optimization Over Random Networks

This paper studies a distributed stochastic optimization problem over random networks with imperfect communications subject to a global constraint, which is the intersection of local constraint sets assigned to agents. The global cost function is the sum of local cost functions, each of which is the expectation of a random cost function. By incorporating the augmented Lagrange technique with the projection method, a stochastic approximation based distributed primal-dual algorithm is proposed to solve the problem. Each agent updates its estimate by using the local observations and the information derived from neighbors. For the constrained problem, the estimates are first shown to be bounded almost surely (a.s.), and then are proved to converge to the optimal solution set a.s. Furthermore, the asymptotic normality and efficiency of the algorithm are addressed for the unconstrained case. The results demonstrate the influence of random networks, communication noises, and gradient errors on the performance of the algorithm. Finally, numerical simulations demonstrate the theoretic results.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{Asymptotic Properties of Primal-Dual Algorithm for Distributed Stochastic Optimization Over Random Networks} 
\newcommand{\TheAuthors}{Jinlong Lei, Han-Fu Chen, and Hai-Tao Fang}

% Sets running headers as well as PDF title and authors
\headers{ Primal-Dual Algorithm for Distributed Stochastic Optimization  }{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors DATA.
\funding{This
work was supported by the NSFC under Grants 61273193, 61120106011, 61134013, 61573345,
the 973 program of China under grant No.2014CB845301, and
the National Center for Mathematics and Interdisciplinary Sciences, Chinese
Academy of Sciences.}}}

% Authors: full names plus addresses.


\author{
  Jinlong Lei, Han-Fu Chen, and Hai-Tao Fang\thanks{The Key Laboratory  of Systems and Control, Academy of
Mathematics and Systems Science, Chinese Academy of Sciences
    (\email{leijinlong11@mails.ucas.ac.cn},  \email{hfchen@iss.ac.cn},  \email{htfang@iss.ac.cn}).}
}

 
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

